Temperature field and heat generation at the tip of a cutout in a viscoelastic solid body undergoing loading

Using the finite element method we quantitatively analyse temperature field evolution in a viscoelastic solid undergoing a loading--unloading process. In particular we investigate the temperature field inside a Kelvin--Voigt type viscoelastic body with a thin cutout. We find that the viscosity significantly contributes to the temperature field changes, and that the temperature field changes initiated by the loading--unloading process are strongly concentrated at the tip of the thin cutout. The predicted temperature field qualitatively corresponds to the temperature field observed in experiments focused on simultaneous heat and strain measurements at the crack tip inside materials such as the filled rubber.

==> vit-prusa-macros-reference-natural.tex <==
\newcommand{\rplacer}{\kappa_0}       % placer, reference configuration
\newcommand{\rrplacer}{\kappa_R}       % placer, reference configuration
\newcommand{\cplacer}{\kappa_t}       % placer, current configuration
\newcommand{\nplacer}{\kappa_{\mathnormal{p}(\mathnormal{t})}}  % placer, natural configuration

\newcommand{\refnat}{\mathrm{RN}} % reference -> natural
\newcommand{\natcur}{\mathrm{NC}} % natural -> current
\newcommand{\refcur}{\mathrm{RC}} % reference -> current

% PRUSA
% \newcommand{\fgradrn}{\ensuremath{\fgrad_{\refnat}}} % deformation gradient, reference -> natural
% \newcommand{\fgradrng}{\ensuremath{\fgrad_{\refnat}}} % deformation gradient, reference -> natural, symbol G

% \newcommand{\gradvlrn}{\ensuremath{\gradvl_{\refnat}}} % velocity gradient, reference -> natural
% \newcommand{\gradsymrn}{\ensuremath{\gradsym_{\refnat}}} % symmetric part of the velocity gradient, reference -> natural
% \newcommand{\gradasymrn}{\ensuremath{\gradasym_{\refnat}}} % skew symmetric part of the velocity gradient, reference -> natural
% \newcommand{\lcgnc}{\ensuremath{\lcg_{\natcur}}} % left Cauchy--Green tensor, natural -> current
% \newcommand{\rcgnc}{\ensuremath{\rcg_{\natcur}}} % right Cauchy--Green tensor, natural -> current

% \newcommand{\fgradnc}{\ensuremath{\fgrad_{\natcur}}} % deformation gradient, natural -> current
% \newcommand{\fgradrc}{\ensuremath{\fgrad_{\refcur}}} % deformation gradient, reference -> current


% MALEK
\newcommand{\fgradrn}{\ensuremath{\fgrad_{\rplacer(\body)\to \nplacer(\body)}}} % deformation gradient, reference -> natural
\newcommand{\fgradrng}{\ensuremath{\tensorq{G}}} % deformation gradient, reference -> natural, symbol G

\newcommand{\gradvlrn}{\ensuremath{\gradvl_{\nplacer}}} % velocity gradient, reference -> natural
\newcommand{\gradsymrn}{\ensuremath{\gradsym_{\nplacer}}} % symmetric part of the velocity gradient, reference -> natural
\newcommand{\gradasymrn}{\ensuremath{\gradasym_{\nplacer}}} % skew symmetric part of the velocity gradient, reference -> natural

\newcommand{\lcgnc}{\ensuremath{\lcg_{\nplacer}}} % left Cauchy--Green tensor, natural -> current
\newcommand{\lcgncc}{\ensuremath{\lcgc_{\nplacer}}} % left Cauchy--Green tensor, natural -> current, components

\newcommand{\rcgnc}{\ensuremath{\rcg_{\nplacer}}} % right Cauchy--Green tensor, natural -> current
\newcommand{\rcgncc}{\ensuremath{\rcgc_{\nplacer}}} % right Cauchy--Green tensor, natural -> current, components

\newcommand{\fgradnc}{\ensuremath{\fgrad_{\nplacer}}} % deformation gradient, natural -> current
\newcommand{\fgradrc}{\ensuremath{\fgrad}} % deformation gradient, reference -> current, components

% OTHER NOTATIONS
\newcommand{\fgradtot}{\ensuremath{\fgrad_{\rrplacer}}} % total deformation gradient

\newcommand{\elastic}{\mathrm{e}} % elastic
\newcommand{\plastic}{\mathrm{p}} % plastic

\newcommand{\fgradel}{\ensuremath{\fgrad_{\elastic}}} % deformation gradient, elastic part
\newcommand{\fgradpl}{\ensuremath{\fgrad_{\plastic}}} % deformation gradient, plastic part

